Local Policy Optimization for Trajectory-Centric Reinforcement Learning

The goal of this paper is to present a method for simultaneous trajectory and local stabilizing policy optimization to generate local policies for trajectory-centric model-based reinforcement learning (MBRL). This is motivated by the fact that global policy optimization for non-linear systems could be a very challenging problem both algorithmically and numerically. However, a lot of robotic manipulation tasks are trajectory-centric, and thus do not require a global model or policy. Due to inaccuracies in the learned model estimates, an open-loop trajectory optimization process mostly results in very poor performance when used on the real system. Motivated by these problems, we try to formulate the problem of trajectory optimization and local policy synthesis as a single optimization problem. It is then solved simultaneously as an instance of nonlinear programming. We provide some results for analysis as well as achieved performance of the proposed technique under some simplifying assumptions.

==> old_section_3b.tex <==
Consider the deviation of the executed trajectory $\tau_N$ from the optimal trajectory $\hat{\tau}_N$, and denote it as $\delta x_k \equiv x_k - \hat{x}_k$ and $\delta X \equiv X - \hat{X}$ accordingly. Then, introduce the local feedback matrix $W$ that regulates the local trajectory deviation $\delta x_k$ and modify the final control policy as $u_k = \hat{u}_k + \pi_W(\delta x_k)$. The actual system dynamics in terms of the introduced trajectory deviation and the newly introduced control policy is then
\begin{equation}
\begin{aligned}
x_{k+1} = f(x_k, u_k)=f(\hat{x}_k + \delta x_k, \hat{u}_k + \pi_W(\delta x_k))
\end{aligned}
\end{equation}The main objective of the paper is to select the time-invariant feedback policy $W$ that provides an open-loop solution $\hat{U}^*$ that is robust with respect to model uncertainty, external perturbation, etc.
The general optimization problem that achieves that is proposed as:
\begin{equation}\label{generalFormulation}
\begin{aligned}
J^* = & \underset{\hat{U}, \hat{X}, W}{min}\; \underset{\delta x_k \in \mathcal{R}_k}{\E}[ J(\hat{X}+\delta X, \hat{U}+\pi_W(\delta x_k)]\\
&\hat{x}_{k+1} = \hat{f}(\hat{x}_k, \hat{u}_k)\\ 
&\delta x_{k+1} =  x_{k+1} - \hat{x}_{k+1}\\
\end{aligned}
\end{equation}where $\mathcal{R}_k \subset \R^{n_x}$ is a set that describes a local region of uncertainty in $\delta x_k$. The crucial difference between the formulation (\ref{generalFormulation}) and (\ref{NLP}) is that (\ref{generalFormulation}) introduces a new decision variable in the form of a local feedback matrix $W$. The introduction of $W$ adds a degree of freedom that is needed to provide local robustness to the optimal trajectory $\tau_N^*$ in case of existing deviation from optimal trajectory $\delta x_k \in \R_k$. The region $\R_k$ can be estimated with some probability given the probability distribution of $\delta x_k$. 



Solving the optimization problem (\ref{generalFormulation}) is difficult for many reasons. The following lemmas and theorem show how to transform (\ref{generalFormulation}) into a tractable optimization problem. It is first shown in Lemma 1 that the error dynamics are locally linear around the optimal trajectory $\hat{\tau}_N$.

\begin{lem}
The trajectory deviation dynamics $\delta x_{k+1} = x_{k+1} - \hat{x}_{k+1}$ approximated locally around the optimal trajectory $\hat{\tau}_N$ are given by
\begin{equation}
\begin{aligned}
\delta x_{k+1} &= A(\hat{x}_k, \hat{u}_k)\cdot \delta x_k + B(\hat{x}_k, \hat{u}_k)\cdot \pi_W(\delta x_k)\\
A(\hat{x}_k, \hat{u}_k) &\equiv \nabla_{ \hat{x}_k} \hat{f}(\hat{x}_k, \hat{u}_k)\\
B(\hat{x}_k, \hat{u}_k) &\equiv  \nabla_{\hat{u}_k} \hat{f}(\hat{x}_k, \hat{u}_k)
\end{aligned}
\end{equation}
\end{lem}
\begin{proof}

Starting from the definition of trajectory deviation and applying first-order Taylor expansion,\begin{equation}
\begin{aligned}
&\delta x_{k+1} = x_{k+1} - \hat{x}_{k+1} = f(x_k, u_k) - \hat{f} (\hat{x}_k, \hat{u}_k)=\hat{f}(x_k, u_k) \\
&+e(x_k, u_k) - \hat{f} (\hat{x}_k, \hat{u}_k) \\ 
&= \hat{f}(\hat{x}_k + \delta x, \hat{u}_k + \pi_W(\delta x_k)) + e(\hat{x}_k+\delta x, \hat{u}_k + \pi_W(\delta x_k)) \\
& - \hat{f} (\hat{x}_k, \hat{u}_k) 
\approx \hat{f}(\hat{x}_k, \hat{u}_k) - \hat{f}(\hat{x}_k, \hat{u}_k) + \nabla_{ \hat{x}_k} \hat{f}(\hat{x}_k, \hat{u}_k)\cdot \delta x_k
\\ 
&+\nabla_{\hat{u}_k} \hat{f}(\hat{x}_k, \hat{u}_k)\cdot \pi_W(\delta x_k) + e(\hat{x}_k+\delta x, \hat{u}_k + \pi_W(\delta x_k))\\
& \approx   A(\hat{x}_k, \hat{u}_k)\cdot \delta x_k + B(\hat{x}_k, \hat{u}_k)\cdot \pi_W(\delta x_k)
\end{aligned}
\end{equation}which proves the statement of this lemma. 
\end{proof}

In the next lemma, the problem (\ref{generalFormulation}) is transformed into a tractable optimization problem at the cost of a more conservative optimal solution compared to the original problem.
\begin{lem} 

Consider the optimization problem 
\begin{equation}\label{newFormulation1}
\begin{aligned}
J^* = & \underset{\hat{U}, \hat{X}}{min} \; [J(\hat{X}, \hat{U})]  + \underset{\hat{U}, \hat{X}, W}{min}\; \underset{\delta x_k \in \mathcal{R}_k}{max}[J (\delta X, \pi_W(\delta X))]\\
&\hat{x}_{k+1} = \hat{f}(\hat{x}_k, \hat{u}_k)\\ 
&\delta x_{k+1} =  x_{k+1} - \hat{x}_{k+1}\\
\end{aligned}
\end{equation}The cost of the optimal solution of (\ref{newFormulation1}) is an upper bound of the optimal cost of (\ref{generalFormulation}).
\end{lem}
\begin{proof}

First notice that the cost function $c(\cdot, \cdot)$ has the property of a norm on the vector space $[x_k^T, u_k^T]^T$. The norm satisfies the triangle inequality $c(a_1+a_2, b_1 + b_2) \leq c(a_1, b_1) + c(a_2, b_2)$, so the following is true: $J(\hat{X}+\delta X, \hat{U}+\pi_W(\delta x_k)) \leq J(\hat{X}, \hat{U}) + J (\delta X, \pi_W(\delta x_k))$. Therefore, the cost function (\ref{generalFormulation}) is upper bounded as
\begin{equation}\label{firstIneq}
\begin{aligned}
&\underset{\hat{U}, \hat{X}, W}{min}\; \underset{\delta x_k \in \mathcal{R}_k}{\E}[ J(\hat{X}+\delta X, \hat{U}+\pi_W(\delta x_k)] \\
\leq 
&\underset{\hat{U}, \hat{X}, W}{min}\; \underset{\delta x_k \in \mathcal{R}_k}{\E}[J(\hat{X}, \hat{U}) + J (\delta X, \pi_W(\delta x_k))] 
\end{aligned}
\end{equation}Next, replace the expectation of the cost function in (\ref{generalFormulation}) with the worst case $\delta x_k \in \mathcal{R}_k$ to find the robust upper bound for (\ref{firstIneq})
\begin{equation}\label{secondIneq}
\begin{aligned}
&\underset{\hat{U}, \hat{X}, W}{min}\; \underset{\delta x_k \in \mathcal{R}_k}{\E}[ J(\hat{X}+\delta X, \hat{U}+\pi_W(\delta x_k))]\\
\leq 
&\underset{\hat{U}, \hat{X}, W}{min}\; \underset{\delta x_k \in \mathcal{R}_k}{\E}[J(\hat{X}, \hat{U}) + J (\delta X, \pi_W(\delta x_k))] \\
\leq 
&\underset{\hat{U}, \hat{X}, W}{min} \;\underset{\delta x_k \in \mathcal{R}_k}{max}\; [J(\hat{X}, \hat{U}) + J (\delta X, \pi_W(\delta x_k))]
\end{aligned}
\end{equation}which results in the optimization problem (\ref{newFormulation1}). 
\end{proof}

Interestingly, the first term in the cost of the optimization problem (\ref{newFormulation1}) is identical to the cost function in (\ref{NLP}), therefore encouraging low cost optimal trajectory. The second term, on the other hand, provides robustness along that trajectory. 

The next theorem shows the final version of the optimization problem that is proposed in this paper.

\begin{thm}
The solution of the optimization problem 
\begin{equation}\label{finalFormulation}
\begin{aligned}
J^* = & \underset{\hat{U}, \hat{X}, \epsilon}{min} \; [J(\hat{X}, \hat{U}) + \underset{k}{\sum}\epsilon_k]  \\
&\hat{x}_{k+1} =  \hat{f}(\hat{x}_k, \hat{u}_k)\\ 
& \underset{\delta x_k \in \mathcal{R}_k}{max}\; \bigg (c \Big (f(\hat{x}_k + \delta x_k, \hat{u}_k + \pi_W(\delta x_k)) \\&- \hat{x}_{k+1},  \pi_W(\delta x_k)\Big )\bigg ) < \epsilon_k \\
\end{aligned}
\end{equation}and the solution to (\ref{newFormulation1}) are equal.
\end{thm}
\begin{proof} Formulate the optimization problem (\ref{newFormulation1}) in epigraph form by transforming the second term in the cost function into $k$ inequalities.
\begin{equation}\label{epigrafApplied}
\begin{aligned}
J^* = & \underset{\hat{U}, \hat{X}, \epsilon_k}{min} \; [J(\hat{X}, \hat{U})  + \underset{k}{\sum}\epsilon_k] \\
&\hat{x}_{k+1} = \hat{f}(\hat{x}_k, \hat{u}_k)\\ 
&\delta x_{k+1} =  x_{k+1} - \hat{x}_{k+1}\\
& \underset{ \delta x_k \in \mathcal{R}_k}{max}[c (\delta x_k, \pi_W(\delta x_k))] \leq \epsilon_k\\
\end{aligned}
\end{equation}Eliminate the second equality constraint in (\ref{epigrafApplied}) and complete the proof by writing the resulting optimization problem as (\ref{finalFormulation}). 
\end{proof}

The problem transformation resulted in a well posed non-linear optimization problem (\ref{finalFormulation}). The inequality constraint introduced in (\ref{finalFormulation}) is referred to as a \textit{robust constraint} in the rest of the paper.

Before moving to the solution approach, it is useful to understand the intuition behind the resulting formulation, as well as its benefits. 

The first point to make is that the optimization problem (\ref{finalFormulation}) enforces robustness in terms of hard inequality constraint by introducing slack variables $\epsilon_k$, as opposed to the previous formulations that enforced it directly in the cost. By introducing slack variables, the cost function (\ref{finalFormulation}) becomes separable in decision variables of the open-loop solution $(\hat{X}, \hat{U})$ and the feedback parameters of controller $W$. With that property, the problem (\ref{finalFormulation}) is receptive of algorithms that take advantage of the separability in the cost (i.e. ADMM).

Secondly, the robust inequality constraint has clear intuition related to trajectory tracking. Since $c(\cdot, \cdot)$ is a norm on vector space, the term
\begin{equation}\label{d}
\begin{aligned}
d(\hat{x}_k, \hat{u}_k, W) \equiv & c \Big (f(\hat{x}_k + \delta x_k, \hat{u}_k + \pi_W(\delta x_k)) \\ &- \hat{x}_{k+1}, \pi_W(\delta x_k)\Big )
\end{aligned}
\end{equation}that appears in the inequality constraint of (\ref{finalFormulation}), can be understood as the tracking error measured in the norm $c(\cdot, \cdot)$. The term
\begin{equation}\label{dmaxgen}
\begin{aligned}
d_{max}(\hat{x}_k, \hat{u}_k, W) \equiv & \underset{\delta x_k \in \mathcal{R}_k}{max}\; \bigg (c \Big (f(\hat{x}_k + \delta x_k, \hat{u}_k + \pi_W(\delta x_k)) \\ & - \hat{x}_{k+1}, \pi_W(\delta x_k)\Big )\bigg )
\end{aligned}
\end{equation}is the worst case of it. Therefore, the optimization problem (\ref{finalFormulation}) simultaneously solves for the optimal trajectory and bounds the trajectory tracking error measured in the norm $c(\cdot, \cdot)$ by enforcing the robust constraint. This constraint satisfaction provides the robustness certificate for the generated optimal trajectory.

In problems of interest, the cost function $c(\cdot, \cdot)$ is often in the form of a weighted $l2$-norm. The uncertainty region $\R_k$ is commonly approximated by fitting ellipsoid to the uncertainty estimate, which can be calculated by using stochastic model learning approaches like Gaussian processes or any other suitable technique. The next corollary shows a special version of the optimization problem (\ref{finalFormulation}), where the region of uncertainty and cost function are chosen according to this paragraph.

\textbf{Corollary 4.}
Assume that the cost function is $c(x,u) = ||x||_q^2 + ||u||_r^2$ and the uncertainty region $\R_k = \{\delta x_k : \delta x_k^T s_k \delta x_k \leq  1\}$, where $q,r,s_k$ are symmetric positive definite matrices. Then (\ref{finalFormulation}) specializes in the following form
\begin{equation}\label{simpleFormulation}
\begin{aligned}
J^* = & \underset{\hat{U}, \hat{X}, \epsilon}{min} \; [J(\hat{X}, \hat{U}) + \underset{k}{\sum}\epsilon_k]  \\
&\hat{x}_{k+1} = \hat{f}(\hat{x}_k, \hat{u}_k)\\ 
&  d_{max}< \epsilon_k \\
\end{aligned}
\end{equation} with
\begin{equation}\label{dmax}
\begin{aligned}
&d_{max} =  \\ 
&\max_{\delta x_k^T s_k \delta x_k \leq  1} ||A(\hat{x}_k, \hat{u}_k)\cdot \delta x_k + B(\hat{x}_k, \hat{u}_k)\cdot \pi_W(\delta x_k)||_q^2
\end{aligned}
\end{equation}
\noindent\textbf{proof}

Apply Lemma 1 to the robust constraint in (\ref{finalFormulation}) and introduce modifications introduced in this corollary to write (\ref{simpleFormulation}). Q.E.D.

